Optimized Portfolio Contracts for Bidding the Cloud

Amazon EC2 provides two most popular pricing schemes--i) the {\em costly} on-demand instance where the job is guaranteed to be completed, and ii) the {\em cheap} spot instance where a job may be interrupted. We consider a user can select a combination of on-demand and spot instances to finish a task. Thus he needs to find the optimal bidding price for the spot-instance, and the portion of the job to be run on the on-demand instance. We formulate the problem as an optimization problem and seek to find the optimal solution. We consider three bidding strategies: one-time requests with expected guarantee and one-time requests with penalty for incomplete job and violating the deadline, and persistent requests. Even without a penalty on incomplete jobs, the optimization problem turns out to be non-convex. Nevertheless, we show that the portion of the job to be run on the on-demand instance is at most half. If the job has a higher execution time or smaller deadline, the bidding price is higher and vice versa. Additionally, the user never selects the on-demand instance if the execution time is smaller than the deadline. The numerical results illustrate the sensitivity of the effective portfolio to several of the parameters involved in the model. Our empirical analysis on the Amazon EC2 data shows that our strategies can be employed on the real instances, where the expected total cost of the proposed scheme decreases over 45\% compared to the baseline strategy.

==> algo.tex <==
\section{Solution Methodology}\label{sec:algo}


==> bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./bio/yang.png}}]{Yang Zhang} obtained her Bachelor's in Information Management and Information Systems from Southeast University in 2014 and is pursuing her Ph.D. in Operations Research, Industrial Engineering at Purdue University. Her research interests are: pricing of cloud systems, dynamic matching in online marketplaces, simulation and optimization. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./bio/arnob.jpg}}]{Arnob Ghosh} received the B.E. degree in Electronics and Telecommunications from Jadavpur University, Kolkata, India in 2011; the PhD and M.S. degree in Electrical Engineering from the University of Pennsylvania in 2016 and 2013 respectively. He is currently a Postdoctoral Research Associate in the Industrial Engg. Department of Purdue University. His research interests are smart grid, economic aspects of spectrum sharing in wireless network, and game theoretic approach for resource allocations in wireless network. He served as a reviewer in {\it IEEE Transactions on Signal Processing}, {\it ACM/IEEE Transactions on Networking}, and {\it IEEE Transactions on Communication}. 
\end{IEEEbiography}
%\balance
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./bio/vaneet.eps}}]{Vaneet Aggarwal (S'08 - M'11 - SM’15)}
	received the B.Tech. degree in 2005 from the Indian Institute of Technology, Kanpur, India, and the M.A. and Ph.D. degrees in 2007 and 2010, respectively from Princeton University, Princeton, NJ, USA, all in Electrical Engineering.
	
	He is currently an Assistant Professor at Purdue University, West Lafayette, IN. Prior to this, he was a Senior Member of Technical Staff Research at AT\&T Labs-Research, NJ, and an Adjunct Assistant Professor at Columbia University, NY. His current research interests are in communications and networking, video streaming, cloud computing, and machine learning. 
	
	Dr. Aggarwal was the recipient of Princeton University's Porter Ogden Jacobus Honorific Fellowship in 2009. In addition, he received AT\&T Key Contributor award in 2013, AT\&T Vice President Excellence Award in 2012, and AT\&T Senior Vice President Excellence Award in 2014. He received the 2017 Jack Neubauer Memorial Award, recognizing the Best Systems Paper published in the IEEE Transactions on Vehicular Technology. He is serving on the editorial board of the {\it IEEE Transactions on Communications} and the {\it IEEE Transactions on Green Communications and Networking.}
\end{IEEEbiography}


==> conclusion.tex <==
\section{Conclusions and Future Work}\label{con}

In this paper, we firstly develop optimization models for cloud users with different strategies: one-time request with/without penalty, and persistent request. We then answer the question of how much of the job should run on spot instance and how much the users should bid for the spot service. In certain cases, we derive closed-form formulas and find analytical expression for the optimal solution. 

 In reality, there is a two-minute warning to the user before the instance is revoked \cite{wang17}. The user can use re-bidding strategy to avoid termination of the job. We do not consider such scenario in this paper, however, we believe that such analysis constitutes an interesting future direction.

\section{Acknowledgment}




\appendices

\section{Proof of ??}

\begin{claim}\label{cla1}
When $t_{s}\leq t_{e} \leq 2t_{s}$, $q^{*} \leq \frac{1}{2} \leq \frac{t_{s}}{t_{e}}$ and $F_\pi(p) \geq \frac{1}{2}$
\end{claim}


\begin{proof}
 Because the on-demand price is no less than spot price,  the "decision maker" wants to run as much job as possible on spot instance such that the total cost is minimized, which means the job on the spot instance will not get stopped until the deadline is met. Also because $t_{e} \leq 2t_{s}$, no less than half of the job will be run on spot instance, i.e., $q^{*} \leq \frac{1}{2} \leq \frac{t_{s}}{t_{e}}$. 


It is clear that $t_{s}F_\pi(p) \geq (1-q)t_{e} \geq \frac{1}{2}t_{e} $. Because $t_{s} \leq t_{e}$, $F_\pi(p) \geq \frac{1}{2}$.
\end{proof}


Proof of Proposition \ref{pro1}
\begin{proof}
$$  q^{*} = 1- \frac{  t_{s}-t_{k}( \frac{1}{F_{\pi}(p^{*})} -1  )   }{t_{e}} $$ on the condition that $0 \leq q^{*} \leq 1$ and $q^{*} \leq \frac{t_{s}}{t_{e}}$.

From Claim \ref{cla1}, we know that the condition $q^{*}\leq \frac{t_{s}}{t_{e}} \leq 1$ always meets. Then we need to prove the the condition $q^{*} \geq 0$ is satisfied. 

Because we assume that $t_{s} \leq t_{e}$, $$q^{*}=1-\frac{t_{s}}{t_{e}}+\frac{t_{k}}{t_{e}}(\frac{1}{F_{\pi}(p)} -1) \geq 1-\frac{t_{s}}{t_{e}} \geq 0$$ as long as $0 \leq F_{\pi}(p) \leq 1$. 
 
Then we substitute $q$ in (P1) with $q^{*}$, (P1)  becomes


\begin{align}
\begin{split}
{\text{(P1') \quad   min}} &
\quad t_{e} \bar{\pi} + [t_{s}-t_{k}(\frac{1}{F_{\pi}(p)}-1)][ \frac{  \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx  }{  F_{\pi}(p) } - \bar{\pi}     ]
  \end{split}
\label{obj1} 
\\[2ex]
\text{subject to}\qquad & t_{s} - t_{k}(\frac{1}{F_{\pi}(p)} -1)\leq \frac{t_{k}}{1-F_{\pi}(p)} 
\label{P1-11} 
\\
& \underline{\pi} \leq  p \leq \bar{\pi}
\label{P1-41}
\end{align}





Suppose
$$G(p) =  t_{e} \bar{\pi} + [t_{s}-t_{k}(\frac{1}{F_{\pi}(p)}-1)][ \frac{  \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx  }{  F_{\pi}(p) } - \bar{\pi}     ]$$

\begin{equation}
\begin{split}
\frac{\partial G(p)}{\partial p}&=\frac{t_{k}f_{\pi}(p)}{F_{\pi}(p)^{2}}[ \frac{  \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx  }{  F_{\pi}(p) } - \bar{\pi} ] \\
&+ \frac{f_{\pi}(p)[pF_{\pi}(p)-\int_{\underline{\pi}}^{p}xf_{\pi}(x)dx]}{F_{\pi}^{2}(p)}[t_{s}-t_{k}(\frac{1}{F_{\pi}(p)}-1)]\\
&=\frac{f_{\pi}(p)}{F_{\pi}(p)^{2}}[  \frac{  \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx  }{  F_{\pi}(p) }t_{k} - \bar{\pi}t_{k} \\
& + (pF_{\pi}(p)-\int_{\underline{\pi}}^{p}xf_{\pi}(x)dx) (t_{s}-t_{k}(\frac{1}{F_{\pi}(p)}-1))    ]
\end{split}
\end{equation}

Suppose $g(p) =  \frac{  \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx  }{  F_{\pi}(p) }t_{k} - \bar{\pi}t_{k}  + (pF_{\pi}(p)-\int_{\underline{\pi}}^{p}xf_{\pi}(x)dx) (t_{s}-t_{k}(\frac{1}{F_{\pi}(p)}-1)) $


\begin{equation}
\begin{split}
&\frac{\partial g(p)}{\partial p} \\
&= \frac{2t_{k}f_{\pi}(p)}{F_{\pi}(p)} ( p - \frac{\int_{\underline{\pi}}^{p}xf_{\pi}(x)dx}{F_{\pi}(p)}   )+ F_{\pi}(p)(t_{s}-t_{k}(\frac{1}{F_{\pi}(p)}-1)) \\
&\geq 0
\end{split}
\end{equation}

Thus $g(p)$ monotonically increases with $p$. So is $\frac{\partial G(p)}{\partial p}$. 

because $\lim_{p \to \underline{\pi} }g(p) = t_{k}\underline{\pi}-t_{k}\bar{\pi} <0 $, and $g(\bar{\pi})=( \bar{\pi}-\int_{\underline{\pi}}^{\bar{\pi}}xf_{\pi}(x)dx )(t_{s}-t_{k})>0$, $\frac{\partial G(p)}{\partial p}$ increases monotonically from a negative value to a positive value, i.e., $G(p)$ first decreases and then increases with $p$. Thus $G(p)$ is minimized when $\frac{\partial G(p)}{\partial p}=0$. Letting $\frac{\partial G(p)}{\partial p} = 0$, we thus deduce 

\begin{equation}
\begin{split}
&\psi_{1}(p) \\
&=\frac{ 2t_{k} \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx  }{  F_{\pi}(p) } + 2pt_{s}F_{\pi}(p) - pt_{s} - (t_{s}+t_{k}) \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx\\
&=  t_{k}\bar{\pi}
\end{split}
\end{equation}

so $\hat{p_{1}}^{*} = \psi_{1}^{-1} (t_{k}\bar{\pi})$. 

Until now, we just consider the objective function and constraint (\ref{P1-41}), next step we will analyse constraint (\ref{P1-11}). 




Constraint (\ref{P1-11}) is equivalent to 

\begin{equation}\label{con111}
M(p) = (t_{s}+t_{k})F_{\pi}(p) - (t_{s}+t_{k})F_{\pi}(p)^{2} - t_{k} \leq 0
\end{equation}


Because $\frac{\partial M(p)}{\partial p} = (t_{s}+t_{k})f_{\pi}(p)(1-2F_{\pi}(p))\leq 0$, $M(p)$ is monotone decreasing with $p$. Also because $\lim_{p: F_{\pi}(p) \to \frac{1}{2}} M(p) \geq 0$ and $M(  \bar{\pi}) \leq 0$, there exists one and only one $\hat{p_{2}}^{*} $ such that $M(\hat{p_{2}}^{*} ) = 0$, so constraint (\ref{P1-11}) ( or (\ref{con111}))is equivalent to 


\begin{equation}\label{con1111}
p \geq \hat{p_{2}}^{*}
\end{equation}

In order to get the optimal solution for (P1'), we need to take the maximum of $ \hat{p_{1}}^{*}$ and $ \hat{p_{2}}^{*}$, i.e., $p^{*}= \max \{  \hat{p_{1}}^{*},  \hat{p_{2}}^{*}   \}$


\end{proof}

Proof of Proposition \ref{pro2}
\begin{proof}
When $t_{s}>t_{e}$, we claim that $q=0$ because the decision maker would like to assign as much job as possible to the spot instance. 

When $q=0$, the objective function of (P1) becomes $$G(p) = \frac{t_{e}  \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx}{F_{\pi}(p)}$$
Then we take the first derivative of $G(p)$ and get $$  \frac{\partial G(p)}{\partial p} =t_{e}f_{\pi}(p)(  \frac{p - \frac{\int_{\underline{\pi}}^{p}xf_{\pi}(x)dx}{F_{\pi}(p)}       }{  F_{\pi}(p)  }   ) \geq 0, $$ which means the $G(p)$ monotonic increasing with $p$.  Minimizing $G(p)$ is equivalent to finding the minimum $p$ in its feasible set. Suppose $t_{s}-t_{e}\geq t_{k}$ and $t_{e}\geq 2t_{k}$, then
 $p = \max\{  F_{\pi}^{-1}(1-\frac{t_{k}}{t_{e}}), F_{\pi}^{-1}(\frac{t_{k}}{t_{s}-t_{e}+t_{k}}), \underline{\pi} \}= F_{\pi}^{-1}(1-\frac{t_{k}}{t_{e}})$.



\end{proof}
















\begin{claim}\label{cla2}
In persistent request, when $\frac{t_{e}}{2} < t_{s} \leq t_{e}$, $F_{\pi}(p) > 0.5$. 
\end{claim}

Proof of Proposition \ref{pro3}
\begin{proof}
When $\frac{t_{e}}{2} < t_{s} < t_{e}$, the decision maker will assign as much job as possible to spot instance to minimize the total cost on the condition that the deadline requirement is met. 

\begin{equation}\label{P3-q}
\begin{split}
q^{*}  =1-\frac{t_{r}+t_{s}F_{\pi}(p)( 1-\frac{t_{r}}{t_{k}}(1-F_{\pi}(p))   )  }{t_{e}}   
\end{split}
\end{equation}

Then substitute $q$ using $q^{*}$ in (P3), we will get a new optimization problem (P3')

\begin{align}
\begin{split}
{\text{(P3') \quad   min}} &
\quad  G(p) = t_{e}\bar{\pi} - t_{r}\bar{\pi} - t_{s}F_{\pi}(p)\bar{\pi}[ 1-\frac{t_{r}}{t_{k}}(1-F_{\pi}(p))] \\
&+t_{s} \int_{\underline{\pi}}^{p}f_{\pi}(x)dx
  \end{split}
\label{green} 
\\
\text{s.t.}\qquad & t_{s}\int_{\underline{\pi}}^{p} xf_{\pi}(x) dx \leq t_{r}\bar{\pi}+t_{s}F_{\pi}(p) \bar{\pi}[1-\frac{t_{r}}{t_{k}}(1-F_{\pi}(p))]
\label{gc0}
\\
&  (1-\frac{t_{r}+t_{s}F_{\pi}(p)( 1-\frac{t_{r}}{t_{k}}(1-F_{\pi}(p))   )  }{t_{e}} ) t_{e} \leq t_{s}
\label{gc1}
\\
& t_{r} < \frac{t_{k}}{1-F_{\pi}(p)}
\label{gc2}
\\
& \underline{\pi} \leq  p \leq \bar{\pi}
\label{gc3}
\\
& 1-\frac{t_{r}+t_{s}F_{\pi}(p)( 1-\frac{t_{r}}{t_{k}}(1-F_{\pi}(p))   )  }{t_{e}}  \geq 0
\label{gc4}
\end{align}

Take the first-order derivative of $G(p)$, we have 
$$ \frac{\partial G(p)}{\partial p}= (p-\bar{\pi})t_{s}f_{\pi}(p) + \frac{t_{r}t_{s}}{t_{k}}\bar{\pi}f_{\pi}(p)(1-2F_{\pi}(p)) <0, $$ so $G(p)$ monotonic decreasing with $p.$ Thus, the optimal solution is $p^{*}= \bar{\pi}$. In addition, the constraints (\ref{gc0}), (\ref{gc1}) and (\ref{gc4}) are satisfied at optimality. 

Substitute $p$ with $p^{*}=\bar{\pi}$ in (\ref{P3-q}), we will get Proposition \ref{pro3}.
\end{proof}


Proof of Proposition \ref{pro4}
\begin{proof}
Similar to the proof of \ref{pro2}, when $t_{s}>t_{e}$, the decision maker will assign the whole job to the spot instance,  i.e., $q=0$. 
When $q = 0$, the objective in (P3) becomes $$\Phi(p) = \frac{ t_{e}-t_{r} }{1-  \frac{t_{r}}{t_{k}} (1-F_{\pi}(p) )   } \frac{ \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx}{F_{\pi}(p)}$$. By taking the first derivative of $\Phi(p)$ above, we will have 

$$\frac{\partial \Phi(p)}{\partial p  } =  \frac{ (t_{e}-t_{r})f_{\pi}(p)( 1-\frac{t_{r}}{t_{k}}+2\frac{t_{r}}{t_{k}}F_{\pi}(p)  )   }{ h(p)^{2}   }g(p)    $$

where 
$$g(p)=-\int_{\underline{\pi}}^{p} x f_{\pi}(x)dx+p \frac{(1-\frac{t_{r}}{t_{k}})F_{\pi}(p)+\frac{t_{r}}{t_{k}}(F_{\pi}(p))^{2} }{1-\frac{t_{r}}{t_{k}}+2\frac{t_{r}}{t_{k}}F_{\pi}(p)}$$

and 
$$
h(p)=(1-\frac{t_{r}}{t_{k}})F_{\pi}(p)+\frac{t_{r}}{t_{k}}(F_{\pi}(p))^{2}
$$

Because $\frac{ (t_{e}-t_{r})f_{\pi}(p)( 1-\frac{t_{r}}{t_{k}}+2\frac{t_{r}}{t_{k}}F_{\pi}(p)  )   }{ h(p)^{2}   }>0$, in order to show the positivity of $\Phi(p)$, we take the first derivative of $g(p)$ and then we have 

$$\frac{\partial g(p)}{\partial p}=\frac{1-\frac{t_{r}}{t_{k}}+2 \frac{t_{r}}{t_{k}}(F_{\pi}(p)-pf_{\pi}(p))}{(1-\frac{t_{r}}{t_{k}}+2\frac{t_{r}}{t_{k}}F_{\pi}(p))^{2} }h(p)$$

Because $F_{\pi}(p)$ is concave and $F_{\pi}(p)-pf_{\pi}(p) \geq 0$, we have $\frac{\partial g(p)}{\partial p} \geq 0$. Thus, $g(p)$     monotonically increases with $p$. By the fact that $g(\underline{\pi})=0$, then $g(p) \geq 0$ and  $\frac{\partial \Phi(p)}{\partial p  } \geq 0 $, i.e., $\Phi(p)$ increases monotonically with $p$. 

In order to minimize the total cost, we just need to choose the lowest feasible bid price. constraint (\ref{green-constraint-1}) is equivalent to $$g(p) =  \frac{t_{r}}{t_{k}}F_{\pi}(p)^{2} + (1- \frac{t_{r}}{t_{k}})F_{\pi}(p) \geq \frac{t_{e}-t_{r}}{t_{s}}$$. It is clear that $g(p)$ monotonically increases with $p$, so we just need to find the minimum value to satisfy constraint (\ref{green-constraint-1}), that is, $g(p^{*})=\frac{t_{e}-t_{r}}{t_{s}}$. Because $0 \leq \frac{t_{e}-t_{r}}{t_{s}} \leq 1$, the maximum and minimum value of $g(p)$ is $g_{max}(p) = g(\bar{\pi})=1 $ and $g_{min}(p) = g(\underline{\pi})=0$ respectively. Therefore, constraint (\ref{P1-4}) is satisfied.  Then we get Proposition \ref{pro4}. 

\end{proof}



==> conclusion_-_Copy.tex <==
\section{Conclusions and Future Work}\label{con}

In this paper, we firstly develop optimization models for cloud users with different strategies under the cloud resource providers' spot price setting proposed in \cite{lz15}. We then answer the question of how much of the job should run on spot instance and how much the users should bid for the spot service. In certain cases, we derive closed-form formulas and find analytical expression for the optimal solution. 



\section{Acknowledgment}




\appendices

\section{Proof of ??}

\begin{claim}\label{cla1}
When $t_{s}\leq t_{e} \leq 2t_{s}$, $q^{*} \leq \frac{1}{2} \leq \frac{t_{s}}{t_{e}}$ and $F_\pi(p) \geq \frac{1}{2}$
\end{claim}


\begin{proof}
 Because the on-demand price is no less than spot price,  the "decision maker" wants to run as much job as possible on spot instance such that the total cost is minimized, which means the job on the spot instance will not stopped until the deadline is met. Also because $t_{e} \leq 2t_{s}$, no less than half of the job will be run on spot instance, i.e., $q^{*} \leq \frac{1}{2} \leq \frac{t_{s}}{t_{e}}$. 


It is clear that $t_{s}F_\pi(p) \geq (1-q)t_{e} \geq \frac{1}{2}t_{e} $, because $t_{s} \leq t_{e}$, $F_\pi(p) \geq \frac{1}{2}$.
\end{proof}


Proof of Proposition \ref{pro1}
\begin{proof}
$$  q^{*} = 1- \frac{  t_{s}-t_{k}( \frac{1}{F_{\pi}(p^{*})} -1  )   }{t_{e}} $$ on the condition that $0 \leq q^{*} \leq 1$ and $q^{*} \leq \frac{t_{s}}{t_{e}}$.

From Claim \ref{cla1}, we know that the condition $q^{*}\leq \frac{t_{s}}{t_{e}} \leq 1$ always meets. Then we need to prove the the condition $q^{*} \geq 0$ is satisfied. 

Because we assume that $t_{s} \leq t_{e}$, $$q^{*}=1-\frac{t_{s}}{t_{e}}+\frac{t_{k}}{t_{e}}(\frac{1}{F_{\pi}(p)} -1) \geq 1-\frac{t_{s}}{t_{e}} \geq 0$$ as long as $0 \leq F_{\pi}(p) \leq 1$. 
 
Then we substitute $q$ in (P1) with $q^{*}$, (P1)  becomes


\begin{align}
\begin{split}
{\text{(P1') \quad   min}} &
\quad t_{e} \bar{\pi} + [t_{s}-t_{k}(\frac{1}{F_{\pi}(p)}-1)][ \frac{  \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx  }{  F_{\pi}(p) } - \bar{\pi}     ]
  \end{split}
\label{obj1} 
\\[2ex]
\text{subject to}\qquad & t_{s} - t_{k}(\frac{1}{F_{\pi}(p)} -1)\leq \frac{t_{k}}{1-F_{\pi}(p)} 
\label{P1-11} 
\\
& \underline{\pi} \leq  p \leq \bar{\pi}
\label{P1-41}
\end{align}





Suppose
$$G(p) =  t_{e} \bar{\pi} + [t_{s}-t_{k}(\frac{1}{F_{\pi}(p)}-1)][ \frac{  \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx  }{  F_{\pi}(p) } - \bar{\pi}     ]$$

\begin{equation}
\begin{split}
\frac{\partial G(p)}{\partial p}&=\frac{t_{k}f_{\pi}(p)}{F_{\pi}(p)^{2}}[ \frac{  \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx  }{  F_{\pi}(p) } - \bar{\pi} ] \\
&+ \frac{f_{\pi}(p)[pF_{\pi}(p)-\int_{\underline{\pi}}^{p}xf_{\pi}(x)dx]}{F_{\pi}^{2}(p)}[t_{s}-t_{k}(\frac{1}{F_{\pi}(p)}-1)]\\
&=\frac{f_{\pi}(p)}{F_{\pi}(p)^{2}}[  \frac{  \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx  }{  F_{\pi}(p) }t_{k} - \bar{\pi}t_{k} \\
& + (pF_{\pi}(p)-\int_{\underline{\pi}}^{p}xf_{\pi}(x)dx) (t_{s}-t_{k}(\frac{1}{F_{\pi}(p)}-1))    ]
\end{split}
\end{equation}

Suppose $g(p) =  \frac{  \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx  }{  F_{\pi}(p) }t_{k} - \bar{\pi}t_{k}  + (pF_{\pi}(p)-\int_{\underline{\pi}}^{p}xf_{\pi}(x)dx) (t_{s}-t_{k}(\frac{1}{F_{\pi}(p)}-1)) $


\begin{equation}
\begin{split}
&\frac{\partial g(p)}{\partial p} \\
&= \frac{2t_{k}f_{\pi}(p)}{F_{\pi}(p)} ( p - \frac{\int_{\underline{\pi}}^{p}xf_{\pi}(x)dx}{F_{\pi}(p)}   )+ F_{\pi}(p)(t_{s}-t_{k}(\frac{1}{F_{\pi}(p)}-1)) \\
&\geq 0
\end{split}
\end{equation}

Thus $g(p)$ monotonically increases with $p$. So is $\frac{\partial G(p)}{\partial p}$. 

because $\lim_{p \to \underline{\pi} }g(p) = t_{k}\underline{\pi}-t_{k}\bar{\pi} <0 $, and $g(\bar{\pi})=( \bar{\pi}-\int_{\underline{\pi}}^{\bar{\pi}}xf_{\pi}(x)dx )(t_{s}-t_{k})>0$, $\frac{\partial G(p)}{\partial p}$ increases monotonically from a negative value to a positive value, i.e., $G(p)$ first decreases and then increases with $p$. Thus $G(p)$ is minimized when $\frac{\partial G(p)}{\partial p}=0$. Letting $\frac{\partial G(p)}{\partial p} = 0$, we thus deduce 

\begin{equation}
\begin{split}
&\psi_{1}(p) \\
&=\frac{ 2t_{k} \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx  }{  F_{\pi}(p) } + 2pt_{s}F_{\pi}(p) - pt_{s} - (t_{s}+t_{k}) \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx\\
&=  t_{k}\bar{\pi}
\end{split}
\end{equation}

so $\hat{p_{1}}^{*} = \psi_{1}^{-1} (t_{k}\bar{\pi})$. 

Until now, we just consider the objective function and constraint (\ref{P1-41}), next step we will analyse constraint (\ref{P1-11}). 




Constraint (\ref{P1-11}) is equivalent to 

\begin{equation}\label{con111}
M(p) = (t_{s}+t_{k})F_{\pi}(p) - (t_{s}+t_{k})F_{\pi}(p)^{2} - t_{k} \leq 0
\end{equation}


Because $\frac{\partial M(p)}{\partial p} = (t_{s}+t_{k})f_{\pi}(p)(1-2F_{\pi}(p))\leq 0$, $M(p)$ is monotone decreasing with $p$. Also because $\lim_{p: F_pi(p) \to \frac{1}{2}} M(p) \geq 0$ and $M(  \bar{\pi}) \leq 0$, there exists one and only one $\hat{p_{2}}^{*} $ such that $M(\hat{p_{2}}^{*} ) = 0$, so constraint (\ref{P1-11}) ( or (\ref{con111}))is equivalent to 


\begin{equation}\label{con1111}
p \geq \hat{p_{2}}^{*}
\end{equation}

In order to get the optimal solution for (P1'), we need to take the maximum of $ \hat{p_{1}}^{*}$ and $ \hat{p_{2}}^{*}$, i.e., $p^{*}= \max \{  \hat{p_{1}}^{*},  \hat{p_{2}}^{*}   \}$


\end{proof}

Proof of Proposition \ref{pro2}
\begin{proof}
When $t_{s}>t_{e}$, we claim that $q=0$ because the decision maker would like to assign as much job as possible to the spot instance. 

When $q=0$, the objective function of (P1) becomes $$G(p) = \frac{t_{e}  \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx}{F_{\pi}(p)}$$
Then we take the first derivative of $G(p)$ and get $$  \frac{\partial G(p)}{\partial p} =t_{e}f_{\pi}(p)(  \frac{p - \frac{\int_{\underline{\pi}}^{p}xf_{\pi}(x)dx}{F_{\pi}(p)}       }{  F_{\pi}(p)  }   ) \geq 0, $$ which means the $G(p)$ monotonic increasing with $p$.  Minimizing $G(p)$ is equivalent to finding the minimum $p$ in its feasible set. Suppose $t_{s}-t_{e}\geq t_{k}$ and $t_{e}\geq 2t_{k}$, then
 $p = \max\{  F_{\pi}^{-1}(1-\frac{t_{k}}{t_{e}}), F_{\pi}^{-1}(\frac{t_{k}}{t_{s}-t_{e}+t_{k}}), \underline{\pi} \}= F_{\pi}^{-1}(1-\frac{t_{k}}{t_{e}})$.



\end{proof}



\begin{lemma}
\begin{equation}
\begin{split}
P_{0}^{K}  &=  c\sum_{i=1}^{K}(t_{\#}- it_{k})F_{\pi}(p)^{i-1}(1-F_{\pi}(p))\\
& =ct_{\#}(1-F_{\pi}(p)^{K}) - ct_{k}\frac{1-F_{\pi}(p)^{K}}{1-F_{\pi}(p)} + ct_{k}KF_{\pi}(p)^{K}
\end{split}
\end{equation}

\begin{proof}
\begin{equation}
\begin{split}
P_{0}^{K} & = c\sum_{i=1}^{K}(t_{\#}- it_{k})F_{\pi}(p)^{i-1}(1-F_{\pi}(p)) \\
&= c(1-F_{\pi}(p))[t_{\#}(1+F_{\pi}(p)+F_{\pi}(p)^{2} ...+F_{\pi}(p)^{K-1})]\\
&-c(1-F_{\pi}(p))t_{k}[ 1+2F_{\pi}(p)+3F_{\pi}(p)^{2}...+KF_{\pi}(p)^{K-1}  ]\\
&=c(1-F_{\pi}(p)) t_{\#} \frac{1-F_{\pi}(p)^{K}}{1-F_{\pi}(p)}-c(1-F_{\pi}(p))t_{k}M
\end{split}
\end{equation}

Where 
\begin{equation}
M =  1+2F_{\pi}(p)+3F_{\pi}(p)^{2}...+KF_{\pi}(p)^{K-1}
\end{equation}

Next Step is to calculate $M$.

\begin{equation}\nonumber 
\begin{split}
M & =  1+2F_{\pi}(p)+3F_{\pi}(p)^{2}...+KF_{\pi}(p)^{K-1}\\
M*F_{\pi}(p) & = \qquad F_{\pi}(p)...+(K-1)F_{\pi}(p)^{K-1}+KF_{\pi}(p)^{K}\\
(1-F_{\pi}(p))*M&=1+F_{\pi}(p)+F_{\pi}(p)^{2}...+F_{\pi}(p)^{K-1}-KF_{\pi}(p)^{K}
\end{split}
\end{equation}

\begin{equation}
M=\frac{1-F_{\pi}(p)^{K}}{(1-F_{\pi}(p))^{2}}-\frac{KF_{\pi}(p)^{K}}{1-F_{\pi}(p)}
\end{equation}
\end{proof}
\end{lemma}

Proof of Theorem 1. 
\begin{proof}
In order to calculate the total penalty, we consider the following three types of cases: 

\textbf{(1). Time Line from 0 to $t_{s}-(1-q)t_{e}+t_{k}$ : the job run on spot instance is just interrupted by the system.}



\begin{itemize}
\item When $t_{m}=0$, then the job can be interrupted after one time period with penalty $cF_{\pi}(p)(t_{\#}-t_{k})(1-F_{\pi}(p))$, after two time periods with penalty $cF_{\pi}(p)^{2}(t_{\#}-2t_{k})(1-F_{\pi}(p))$, ... after $(K-1)$ time periods with penalty $cF_{\pi}(p)^{K-1}(t_{\#}-(K-1)t_{k})(1-F_{\pi}(p))$. The total penalty in that case is: $c \sum_{i=1}^{K-1}F_{\pi}(p)^{i}(t_{\#}-it_{k})(1-F_{\pi}(p))$
\item When $t_{m}=t_{k}$, then the job can be interrupted after one time period with penalty $c(1-F_{\pi}(p))F_{\pi}(p)(t_{\#}-t_{k})(1-F_{\pi}(p))$, after two time periods with penalty $c(1-F_{\pi}(p))F_{\pi}(p)^{2}(t_{\#}-2t_{k})(1-F_{\pi}(p))$, ... after $(K-1)$ time periods with penalty $c(1-F_{\pi}(p))F_{\pi}(p)^{K-1}(t_{\#}-(K-1)t_{k})(1-F_{\pi}(p))$. The total penalty in that case is: $c(1-F_{\pi}(p)) \sum_{i=1}^{K-1}F_{\pi}(p)^{i}(t_{\#}-it_{k})(1-F_{\pi}(p))$
\item ...
\item When $t_{m} = t_{s}-(1-q)t_{e}=t_{s}-t_{\#}$, ...The total penalty in that case is: $c(1-F_{\pi}(p))^{\frac{t_{s}-(1-q)t_{e}}{t_{k}}} \sum_{i=1}^{K-1}F_{\pi}(p)^{i}(t_{\#}-it_{k})(1-F_{\pi}(p))$
\end{itemize}

Considering the above possibilities in (1), the total penalty is: 

\begin{equation}
\begin{split}
P_{1} & = c[1+(1-F_{\pi}(p))+(1-F_{\pi}(p))^{2}...\\
&+(1-F_{\pi}(p))^{\frac{t_{s}-(1-q)t_{e}}{t_{k}}}]\sum_{i=1}^{K-1}F_{\pi}(p)^{i}(t_{\#}-it_{k})(1-F_{\pi}(p)) \\
&=  c\frac{1-(1-F_{\pi}(p))^{\frac{t_{s}-(1-q)t_{e}}{t_{k}}+1}}{F_{\pi}(p)} \sum_{i=1}^{K}F_{\pi}(p)^{i}(t_{\#}-it_{k})(1-F_{\pi}(p)) \\
&= c(1-(1-F_{\pi}(p))^{\frac{t_{s}-(1-q)t_{e}}{t_{k}}+1}) P_{0}^{K}
\end{split}
\end{equation}


\textbf{(2). Time Line from $t_{s}-(1-q)t_{e}+t_{k}$ to $t_{s}$: the job run on spot instance can be interrupted by the system or the deadline}
\begin{itemize}
\item When $t_{m}=t_{s}-(1-q)t_{e}+t_{k}$, then the job can be interrupted after one time period with penalty $(1-F_{\pi}(p))^{ \frac{t_{s}-(1-q)t_{e}}{t_{k}} +1}cF_{\pi}(p)(t_{\#}-t_{k})(1-F_{\pi}(p))$, after two time periods with penalty $(1-F_{\pi}(p))^{ \frac{t_{s}-(1-q)t_{e}}{t_{k}} +1}cF_{\pi}(p)^{2}(t_{\#}-2t_{k})(1-F_{\pi}(p))$, ... however, after $(K-1)$ time periods, no matter whether the job is interrupted by the system or not, the job should stop because of the deadline, where the penalty is $(1-F_{\pi}(p))^{ \frac{t_{s}-(1-q)t_{e}}{t_{k}} +1}cF_{\pi}(p)^{K-1}t_{k}$
So  when $t_{m}=t_{s}-(1-q)t_{e}+t_{k}$, the total penalty is 

\begin{equation}
\begin{split}
S_{1} & =[\sum_{i = 1}^{K-1} F_{\pi}(p)^{i}(t_{\#}-it_{k})(1-F_{\pi}(p))c + F_{\pi}(p)^{K}t_{k}c    ]\\
&*(1-F_{\pi}(p))^{\frac{(t_{s}-t_{\#})}{t_{k}}+1}\\
&=  [ F_{\pi}(p)P_{0}^{K-1} +  F_{\pi}(p)^{K}t_{k}c  ](1-F_{\pi}(p))^{\frac{(t_{s}-t_{\#})}{t_{k}}+1}
\end{split}
\end{equation}



\item When $t_{m}=t_{s}-(1-q)t_{e}+2t_{k}$, then the job can be interrupted after one time period with penalty $(1-F_{\pi}(p))^{ \frac{t_{s}-(1-q)t_{e}}{t_{k}} +2}cF_{\pi}(p)(t_{\#}-t_{k})(1-F_{\pi}(p))$, after two time periods with penalty $(1-F_{\pi}(p))^{ \frac{t_{s}-(1-q)t_{e}}{t_{k}} +2}cF_{\pi}(p)^{2}(t_{\#}-2t_{k})(1-F_{\pi}(p))$, ... however, after $(K-2)$ time periods, no matter whether the job is interrupted by the system or not, the job should stop because of the deadline, where the penalty is $(1-F_{\pi}(p))^{ \frac{t_{s}-(1-q)t_{e}}{t_{k}} +2}cF_{\pi}(p)^{K-2}2t_{k}$

\begin{equation}
\begin{split}
S_{2} & = [\sum_{i = 1}^{K-2} F_{\pi}(p)^{i}(t_{\#}-it_{k})(1-F_{\pi}(p))c + F_{\pi}(p)^{K-1}2t_{k}c    ]\\
& *(1-F_{\pi}(p))^{\frac{(t_{s}-t_{\#})}{t_{k}}+2}  \\
&=  [ F_{\pi}(p)P_{0}^{K-2} + F_{\pi}(p)^{K-1}2t_{k}c    ](1-F_{\pi}(p))^{\frac{(t_{s}-t_{\#})}{t_{k}}+2}
\end{split}
\end{equation}



\item ...
\item When $t_{m}= t_{s}-t_{k}$, then no matter the job is interrupted by the system or not, the job should stop because of the deadline, where the penalty is 

\begin{equation}
\begin{split}
S_{K-1} & = (1-F_{\pi}(p))^{ \frac{t_{s}-t_{k}}{t_{k}} }cF_{\pi}(p)(t_{\#}-t_{k})  \\
&=  [F_{\pi}(p)P_{0}^{1} + F_{\pi}(p)^{2}(t_{\#}-t_{k})c](1-F_{\pi}(p))^{\frac{t_{s}}{t_{k}}-1}
\end{split}
\end{equation}

\end{itemize}


Note that 

$$P_{0}^{K}  =Kt_{k}-\frac{ct_{k}}{1-F_{\pi}(p)}+\frac{ ct_{k}F_{\pi}(p)^{K}  }{1-F_{\pi}(p)}$$

Considering the above possibilities in (2), the total penalty is:

\begin{equation}
\begin{split}
P_{2} & =S_{1}+S_{2}...+S_{K-1}   \\
& = F_{\pi}(p) (1-F_{\pi}(p))^{  \frac{t_{s} - t_{\#}}{t_{k}}   }\sum_{i = 1}^{K-1}c t_{\#}(1-F_{\pi}(p)  )^{i} \\
& + F_{\pi}(p)(1-F_{\pi}(p))^{ \frac{   t_{s}-t_{\#}}{t_{k}}}(-\frac{ct_{k}}{1-F_{\pi}(p)}) \sum_{i=1}^{K-1} (1-F_{\pi}(p))^{i}+ \\
& F_{\pi}(p)(1-F_{\pi}(p))^{ \frac{   t_{s}-t_{\#}}{t_{k}}}(\frac{ct_{k}}{1-F_{\pi}(p)}) \sum_{i=1}^{K-1} F_{\pi}(p)^{K}(\frac{1-F_{\pi}(p)}{F_{\pi}(p)} )^{i}\\
& -  F_{\pi}(p) (1-F_{\pi}(p))^{  \frac{t_{s} - t_{\#}}{t_{k}}   }\sum_{i = 1}^{K-1}cit_{k}F_{\pi}(p)^{K}( \frac{1-F_{\pi}(p)}{F_{\pi}(p)}  )^{i}\\
&  +(1-F_{\pi}(p))^{  \frac{t_{s} - t_{\#}}{t_{k}}   }ct_{k}F_{\pi}(p)^{K+1} \sum_{i=1}^{K-1}i ( \frac{1-F_{\pi}(p)}{F_{\pi}(p)}  )^{i}\\
& = cF_{\pi}(p)(1-F_{\pi}(p))^{\frac{t_{s}-t_{\#}}{t_{k}}}(t_{\#}- \frac{t_{k}}{1-F_{\pi}(p)})\sum_{i = 1}^{K-1}(1-F_{\pi}(p)  )^{i} \\
& + cF_{\pi}(p)(1-F_{\pi}(p))^{\frac{t_{s}-t_{\#}}{t_{k}}}F_{\pi}(p)^{K} \frac{t_{k}}{1-F_{\pi}(p)}\sum_{i=1}^{K-1}( \frac{1-F_{\pi}(p)}{F_{\pi}(p)}  )^{i}\\
& =  c(1-F_{\pi}(p))^{\frac{t_{s}-t_{\#}}{t_{k}}}(t_{\#}- \frac{t_{k}}{1-F_{\pi}(p)})[  1-F_{\pi}(p) - (1-F_{\pi}(p))^{K}  ]\\
& + c(1-F_{\pi}(p))^{\frac{t_{s}-t_{\#}}{t_{k}}}F_{\pi}(p)^{2}\frac{t_{k}}{1-F_{\pi}(p)}\\
&* \frac{ (1-F_{\pi}(p))F_{\pi}(p)^{K-1}-(1-F_{\pi}(p))^{K}  }{2F_{\pi}(p) -1}\\
& = c(1-F_{\pi}(p))^{\frac{t_{s}-t_{\#}}{t_{k}}}[  t_{\#} ( 1-F_{\pi}(p) - (1-F_{\pi}(p))^{K}   ) \\
& +t_{k} \frac{F_{\pi}(p)^{K+1}}{2F_{\pi}(p) -1}-t_{k} - t_{k} \frac{ (1-F_{\pi}(p))^{K+1}  }{2F_{\pi}(p) -1} ]
\end{split}
\end{equation}


\textbf{(3). Time Line from $t_{s}$ to $+\infty$: the job run on spot instance can not be started}

Because after $t_{s}$, the job will not be started because of the deadline, the total penalty is $$P_{3}= (1-F_{\pi}(p))^{ \frac{t_{s}}{t_{k}}    }c(1-q)t_{e}.$$

The total penalty is $P = P(1) + P(2) + P(3)$.
After some basic calculation, we can get (\ref{penalty}). 
\end{proof}

\begin{claim}\label{cla2}
In persistent request, when $\frac{t_{e}}{2} < t_{s} \leq t_{e}$, $F_{\pi}(p) > 0.5$. 
\end{claim}

Proof of Proposition \ref{pro3}
\begin{proof}
When $\frac{t_{e}}{2} < t_{s} \leq t_{e}$, the decision maker will assign as much job as possible to spot instance to minimize the total cost on the condition that the deadline requirement is met. 

\begin{equation}\label{P3-q}
\begin{split}
q^{*}  =1-\frac{t_{r}+t_{s}F_{\pi}(p)( 1-\frac{t_{r}}{t_{k}}(1-F_{\pi}(p))   )  }{t_{e}}   
\end{split}
\end{equation}

Then substitute $q$ using $q^{*}$ in (P3), we will get a new optimization problem (P3')

\begin{align}
\begin{split}
{\text{(P3') \quad   min}} &
\quad  G(p) = t_{e}\bar{\pi} - t_{r}\bar{\pi} - t_{s}F_{\pi}(p)\bar{\pi}[ 1-\frac{t_{r}}{t_{k}}(1-F_{\pi}(p))] \\
&+t_{s} \int_{\underline{\pi}}^{p}f_{\pi}(x)dx
  \end{split}
\label{green} 
\\
\text{s.t.}\qquad & t_{s}\int_{\underline{\pi}}^{p} xf_{\pi}(x) dx \leq t_{r}\bar{\pi}+t_{s}F_{\pi}(p) \bar{\pi}[1-\frac{t_{r}}{t_{k}}(1-F_{\pi}(p))]
\label{gc0}
\\
&  (1-\frac{t_{r}+t_{s}F_{\pi}(p)( 1-\frac{t_{r}}{t_{k}}(1-F_{\pi}(p))   )  }{t_{e}} ) t_{e} \leq t_{s}
\label{gc1}
\\
& t_{r} < \frac{t_{k}}{1-F_{\pi}(p)}
\label{gc2}
\\
& \underline{\pi} \leq  p \leq \bar{\pi}
\label{gc3}
\\
& 1-\frac{t_{r}+t_{s}F_{\pi}(p)( 1-\frac{t_{r}}{t_{k}}(1-F_{\pi}(p))   )  }{t_{e}}  \geq 0
\label{gc4}
\end{align}

Take the first-order derivative of $G(p)$, we have 
$$ \frac{\partial G(p)}{\partial p}= (p-\bar{\pi})t_{s}f_{\pi}(p) + \frac{t_{r}t_{s}}{t_{k}}\bar{\pi}f_{\pi}(p)(1-2F_{\pi}(p)) <0, $$ so $G(p)$ monotonic decreasing with $p.$ Thus, the optimal solution is $p^{*}= \bar{\pi}$. In addition, the constraints (\ref{gc0}), (\ref{gc1}) and (\ref{gc4}) are satisfied at optimality. 

Substitute $p$ with $p^{*}=\bar{\pi}$ in (\ref{P3-q}), we will get Proposition \ref{pro3}.
\end{proof}


Proof of Proposition \ref{pro4}
\begin{proof}
Similar to the proof of \ref{pro2}, when $t_{s}>t_{e}$, the decision maker will assign the whole job to the spot instance,  i.e., $q=0$. 
\end{proof}



==> conclusion__1.tex <==
\section{Conclusions and Future Work}\label{con}

In this paper, we firstly develop optimization models for cloud users with different strategies under the cloud resource providers' spot price setting proposed in \cite{lz15}. We then answer the question of how much of the job should run on spot instance and how much the users should bid for the spot service. In certain cases, we derive closed-form formulas and find analytical expression for the optimal solution. 



\section{Acknowledgment}




\appendices

\section{Proof of ??}

\begin{claim}\label{cla1}
When $t_{s}\leq t_{e} \leq 2t_{s}$, $q^{*} \leq \frac{1}{2} \leq \frac{t_{s}}{t_{e}}$ and $ t_{s} - t_{k}( \frac{1}{F_{\pi}(p)}-1) \leq \frac{t_{k}}{1-F_{\pi}(p)} $. 
\end{claim}


\begin{proof}
 Because the on-demand price is no less than spot price,  the "decision maker" wants to run as much job as possible on spot instance such that the total cost is minimized, which means the job on the spot instance will not stopped until the deadline is met. Also because $t_{e} \leq 2t_{s}$, no less than half of the job will be run on spot instance, i.e., $q^{*} \leq \frac{1}{2} \leq \frac{t_{s}}{t_{e}}$. 




The running time of the job before deadline is the difference between deadline and expected time to enter the system, which should be smaller than the expected amount of time that the job will continue running without being interrupted. 
\end{proof}


Proof of Proposition \ref{pro1}
\begin{proof}
First we will prove $q^{*}$.
When $t_{s} \leq t_{e}$, we fix $p = p^{*}$, 
\begin{equation}
\begin{split}
G(p^{*}, q) & = q t_{e}\bar{\pi} + \frac{ (1- q)t_{e}  \int_{\underline{\pi}}^{p^{*}}x f_{\pi}(x)dx}{F_{\pi}(p^{*})} \\
&=\frac{ t_{e}  \int_{\underline{\pi}}^{p^{*}}x f_{\pi}(x)dx}{F_{\pi}(p^{*})} + qt_{e}(\bar{\pi} - \frac{  \int_{\underline{\pi}}^{p^{*}}x f_{\pi}(x)dx}{F_{\pi}(p^{*})}  ) \\
\end{split}
\end{equation}

Because $(\bar{\pi} - \frac{  \int_{\underline{\pi}}^{p^{*}}x f_{\pi}(x)dx}{F_{\pi}(p^{*})}  ) >0 $,  $G(p^{*}, q)$ is monotone increasing, we just need to get the minimum $q$ in its feasible set. 

$q^{*}=\max\{ 1-\frac{t_{k}}{t_{e}(1-F_{\pi}(p^{*}))}, 1- \frac{  t_{s}-t_{k}( \frac{1}{F_{\pi}(p^{*})} -1  )   }{t_{e}}  \}$ on the condition that $0 \leq q^{*} \leq 1$ and $q^{*} \leq \frac{t_{s}}{t_{e}}$

%Because $t_{s} \leq \frac{t_{k}}{1-F_{\pi}(p)}$,
%\begin{equation}
%\begin{split}
% &  \frac{  t_{s}-t_{k}( \frac{1}{F_{\pi}(p^{*})} -1  )   }{t_{e}}  \\
%\leq &  \frac{ \frac{t_{k}}{1-F_{\pi}(p^{*})}-t_{k}( \frac{1}{F_{\pi}(p^{*})} -1  )   }{t_{e}}  \\
%\leq &   \frac{t_{k}}{t_{e}(1-F_{\pi}(p^{*}))} 
%\end{split}
%\end{equation}

From Claim \ref{cla1}, we will get 

$$   1- \frac{  t_{s}-t_{k}( \frac{1}{F_{\pi}(p^{*})} -1  )   }{t_{e}}  \geq  1-\frac{t_{k}}{t_{e}(1-F_{\pi}(p^{*}))}   $$
So $$  q^{*} = 1- \frac{  t_{s}-t_{k}( \frac{1}{F_{\pi}(p^{*})} -1  )   }{t_{e}} $$ on the condition that $0 \leq q^{*} \leq 1$ and $q^{*} \leq \frac{t_{s}}{t_{e}}$.

From Claim \ref{cla1}, we know that the condition $q^{*}\leq \frac{t_{s}}{t_{e}} \leq 1$ always meets. Then we need to proove the the condition $q^{*} \geq 0$ is satisfied. 

Because we assume that $t_{s} \leq t_{e}$, $$q^{*}=1-\frac{t_{s}}{t_{e}}+\frac{t_{k}}{t_{e}}(\frac{1}{F_{\pi}(p)} -1) \geq 1-\frac{t_{s}}{t_{e}} \geq 0$$ as long as $0 \leq F_{\pi}(p) \leq 1$. 
 
Then we substitute $q$ in the objective of (P1) with $q^{*}$, the objective becomes
$$G(p) =  t_{e} \bar{\pi} + [t_{s}-t_{k}(\frac{1}{F_{\pi}(p)}-1)][ \frac{  \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx  }{  F_{\pi}(p) } - \bar{\pi}     ]$$

\begin{equation}
\begin{split}
\frac{\partial G(p)}{\partial p}&=\frac{t_{k}f_{\pi}(p)}{F_{\pi}(p)^{2}}[ \frac{  \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx  }{  F_{\pi}(p) } - \bar{\pi} ] \\
&+ \frac{f_{\pi}(p)[pF_{\pi}(p)-\int_{\underline{\pi}}^{p}xf_{\pi}(x)dx]}{F_{\pi}^{2}(p)}[t_{s}-t_{k}(\frac{1}{F_{\pi}(p)}-1)]\\
&=\frac{f_{\pi}(p)}{F_{\pi}(p)^{2}}[  \frac{  \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx  }{  F_{\pi}(p) }t_{k} - \bar{\pi}t_{k} \\
& + (pF_{\pi}(p)-\int_{\underline{\pi}}^{p}xf_{\pi}(x)dx) (t_{s}-t_{k}(\frac{1}{F_{\pi}(p)}-1))    ]
\end{split}
\end{equation}

Suppose $g(p) =  \frac{  \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx  }{  F_{\pi}(p) }t_{k} - \bar{\pi}t_{k}  + (pF_{\pi}(p)-\int_{\underline{\pi}}^{p}xf_{\pi}(x)dx) (t_{s}-t_{k}(\frac{1}{F_{\pi}(p)}-1)) $


\begin{equation}
\begin{split}
&\frac{\partial g(p)}{\partial p} \\
&= \frac{2t_{k}f_{\pi}(p)}{F_{\pi}(p)} ( p - \frac{\int_{\underline{\pi}}^{p}xf_{\pi}(x)dx}{F_{\pi}(p)}   )+ F_{\pi}(p)(t_{s}-t_{k}(\frac{1}{F_{\pi}(p)}-1)) \\
&\geq 0
\end{split}
\end{equation}

Thus $g(p)$ monotonically increases with $p$. So is $\frac{\partial G(p)}{\partial p}$. 

because $\lim_{p \to \underline{\pi} }g(p) = t_{k}\underline{\pi}-t_{k}\bar{\pi} <0 $, and $g(\bar{\pi})=( \bar{\pi}-\int_{\underline{\pi}}^{\bar{\pi}}xf_{\pi}(x)dx )(t_{s}-t_{k})>0$, $\frac{\partial G(p)}{\partial p}$ increases monotonically from a negative value to a positive value, i.e., $G(p)$ first decreases and then increases with $p$. Thus $G(p)$ is convex in $p$ and is minimized when $\frac{\partial G(p)}{\partial p}=0$. Letting $\frac{\partial G(p)}{\partial p} = 0$, we thus deduce 

\begin{equation}
\begin{split}
&\psi_{1}(p) \\
&=\frac{ 2t_{k} \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx  }{  F_{\pi}(p) } + 2pt_{s}F_{\pi}(p) - pt_{s} - (t_{s}+t_{k}) \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx\\
&=  t_{k}\bar{\pi}
\end{split}
\end{equation}

so $p^{*} = \psi_{1}^{-1} (t_{k}\bar{\pi})$. 
\end{proof}

Proof of Proposition \ref{pro2}
\begin{proof}
When $t_{s}>t_{e}$, we claim that $q=0$ because the decision maker would like to assign as much job as possible to the spot instance. 

When $q=0$, the objective function of (P1) becomes $$G(p) = \frac{t_{e}  \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx}{F_{\pi}(p)}$$
Then we take the first derivative of $G(p)$ and get $$  \frac{\partial G(p)}{\partial p} =t_{e}f_{\pi}(p)(  \frac{p - \frac{\int_{\underline{\pi}}^{p}xf_{\pi}(x)dx}{F_{\pi}(p)}       }{  F_{\pi}(p)  }   ) \geq 0, $$ which means the $G(p)$ monotonic increasing with $p$.  Minimizing $G(p)$ is equivalent to finding the minimum $p$ in its feasible set. Suppose $t_{s}-t_{e}\geq t_{k}$ and $t_{e}\geq 2t_{k}$, then
 $p = \max\{  F_{\pi}^{-1}(1-\frac{t_{k}}{t_{e}}), F_{\pi}^{-1}(\frac{t_{k}}{t_{s}-t_{e}+t_{k}}), \underline{\pi} \}= F_{\pi}^{-1}(1-\frac{t_{k}}{t_{e}})$.



\end{proof}



\begin{lemma}
\begin{equation}
\begin{split}
P_{0}^{K}  &=  c\sum_{i=1}^{K}(t_{\#}- it_{k})F_{\pi}(p)^{i-1}(1-F_{\pi}(p))\\
& =ct_{\#}(1-F_{\pi}(p)^{K}) - ct_{k}\frac{1-F_{\pi}(p)^{K}}{1-F_{\pi}(p)} + ct_{k}KF_{\pi}(p)^{K}
\end{split}
\end{equation}

\begin{proof}
\begin{equation}
\begin{split}
P_{0}^{K} & = c\sum_{i=1}^{K}(t_{\#}- it_{k})F_{\pi}(p)^{i-1}(1-F_{\pi}(p)) \\
&= c(1-F_{\pi}(p))[t_{\#}(1+F_{\pi}(p)+F_{\pi}(p)^{2} ...+F_{\pi}(p)^{K-1})]\\
&-c(1-F_{\pi}(p))t_{k}[ 1+2F_{\pi}(p)+3F_{\pi}(p)^{2}...+KF_{\pi}(p)^{K-1}  ]\\
&=c(1-F_{\pi}(p)) t_{\#} \frac{1-F_{\pi}(p)^{K}}{1-F_{\pi}(p)}-c(1-F_{\pi}(p))t_{k}M
\end{split}
\end{equation}

Where 
\begin{equation}
M =  1+2F_{\pi}(p)+3F_{\pi}(p)^{2}...+KF_{\pi}(p)^{K-1}
\end{equation}

Next Step is to calculate $M$.

\begin{equation}\nonumber 
\begin{split}
M & =  1+2F_{\pi}(p)+3F_{\pi}(p)^{2}...+KF_{\pi}(p)^{K-1}\\
M*F_{\pi}(p) & = \qquad F_{\pi}(p)...+(K-1)F_{\pi}(p)^{K-1}+KF_{\pi}(p)^{K}\\
(1-F_{\pi}(p))*M&=1+F_{\pi}(p)+F_{\pi}(p)^{2}...+F_{\pi}(p)^{K-1}-KF_{\pi}(p)^{K}
\end{split}
\end{equation}

\begin{equation}
M=\frac{1-F_{\pi}(p)^{K}}{(1-F_{\pi}(p))^{2}}-\frac{KF_{\pi}(p)^{K}}{1-F_{\pi}(p)}
\end{equation}
\end{proof}
\end{lemma}

Proof of Theorem 1. 
\begin{proof}
In order to calculate the total penalty, we consider the following three types of cases: 

\textbf{(1). Time Line from 0 to $t_{s}-(1-q)t_{e}+t_{k}$ : the job run on spot instance is just interrupted by the system.}



\begin{itemize}
\item When $t_{m}=0$, then the job can be interrupted after one time period with penalty $cF_{\pi}(p)(t_{\#}-t_{k})(1-F_{\pi}(p))$, after two time periods with penalty $cF_{\pi}(p)^{2}(t_{\#}-2t_{k})(1-F_{\pi}(p))$, ... after $(K-1)$ time periods with penalty $cF_{\pi}(p)^{K-1}(t_{\#}-(K-1)t_{k})(1-F_{\pi}(p))$. The total penalty in that case is: $c \sum_{i=1}^{K-1}F_{\pi}(p)^{i}(t_{\#}-it_{k})(1-F_{\pi}(p))$
\item When $t_{m}=t_{k}$, then the job can be interrupted after one time period with penalty $c(1-F_{\pi}(p))F_{\pi}(p)(t_{\#}-t_{k})(1-F_{\pi}(p))$, after two time periods with penalty $c(1-F_{\pi}(p))F_{\pi}(p)^{2}(t_{\#}-2t_{k})(1-F_{\pi}(p))$, ... after $(K-1)$ time periods with penalty $c(1-F_{\pi}(p))F_{\pi}(p)^{K-1}(t_{\#}-(K-1)t_{k})(1-F_{\pi}(p))$. The total penalty in that case is: $c(1-F_{\pi}(p)) \sum_{i=1}^{K-1}F_{\pi}(p)^{i}(t_{\#}-it_{k})(1-F_{\pi}(p))$
\item ...
\item When $t_{m} = t_{s}-(1-q)t_{e}=t_{s}-t_{\#}$, ...The total penalty in that case is: $c(1-F_{\pi}(p))^{\frac{t_{s}-(1-q)t_{e}}{t_{k}}} \sum_{i=1}^{K-1}F_{\pi}(p)^{i}(t_{\#}-it_{k})(1-F_{\pi}(p))$
\end{itemize}

Considering the above possibilities in (1), the total penalty is: 

\begin{equation}
\begin{split}
P_{1} & = c[1+(1-F_{\pi}(p))+(1-F_{\pi}(p))^{2}...\\
&+(1-F_{\pi}(p))^{\frac{t_{s}-(1-q)t_{e}}{t_{k}}}]\sum_{i=1}^{K-1}F_{\pi}(p)^{i}(t_{\#}-it_{k})(1-F_{\pi}(p)) \\
&=  c\frac{1-(1-F_{\pi}(p))^{\frac{t_{s}-(1-q)t_{e}}{t_{k}}+1}}{F_{\pi}(p)} \sum_{i=1}^{K}F_{\pi}(p)^{i}(t_{\#}-it_{k})(1-F_{\pi}(p)) \\
&= c(1-(1-F_{\pi}(p))^{\frac{t_{s}-(1-q)t_{e}}{t_{k}}+1}) P_{0}^{K}
\end{split}
\end{equation}


\textbf{(2). Time Line from $t_{s}-(1-q)t_{e}+t_{k}$ to $t_{s}$: the job run on spot instance can be interrupted by the system or the deadline}
\begin{itemize}
\item When $t_{m}=t_{s}-(1-q)t_{e}+t_{k}$, then the job can be interrupted after one time period with penalty $(1-F_{\pi}(p))^{ \frac{t_{s}-(1-q)t_{e}}{t_{k}} +1}cF_{\pi}(p)(t_{\#}-t_{k})(1-F_{\pi}(p))$, after two time periods with penalty $(1-F_{\pi}(p))^{ \frac{t_{s}-(1-q)t_{e}}{t_{k}} +1}cF_{\pi}(p)^{2}(t_{\#}-2t_{k})(1-F_{\pi}(p))$, ... however, after $(K-1)$ time periods, no matter whether the job is interrupted by the system or not, the job should stop because of the deadline, where the penalty is $(1-F_{\pi}(p))^{ \frac{t_{s}-(1-q)t_{e}}{t_{k}} +1}cF_{\pi}(p)^{K-1}t_{k}$
So  when $t_{m}=t_{s}-(1-q)t_{e}+t_{k}$, the total penalty is 

\begin{equation}
\begin{split}
S_{1} & =[\sum_{i = 1}^{K-1} F_{\pi}(p)^{i}(t_{\#}-it_{k})(1-F_{\pi}(p))c + F_{\pi}(p)^{K}t_{k}c    ]\\
&*(1-F_{\pi}(p))^{\frac{(t_{s}-t_{\#})}{t_{k}}+1}\\
&=  [ F_{\pi}(p)P_{0}^{K-1} +  F_{\pi}(p)^{K}t_{k}c  ](1-F_{\pi}(p))^{\frac{(t_{s}-t_{\#})}{t_{k}}+1}
\end{split}
\end{equation}



\item When $t_{m}=t_{s}-(1-q)t_{e}+2t_{k}$, then the job can be interrupted after one time period with penalty $(1-F_{\pi}(p))^{ \frac{t_{s}-(1-q)t_{e}}{t_{k}} +2}cF_{\pi}(p)(t_{\#}-t_{k})(1-F_{\pi}(p))$, after two time periods with penalty $(1-F_{\pi}(p))^{ \frac{t_{s}-(1-q)t_{e}}{t_{k}} +2}cF_{\pi}(p)^{2}(t_{\#}-2t_{k})(1-F_{\pi}(p))$, ... however, after $(K-2)$ time periods, no matter whether the job is interrupted by the system or not, the job should stop because of the deadline, where the penalty is $(1-F_{\pi}(p))^{ \frac{t_{s}-(1-q)t_{e}}{t_{k}} +2}cF_{\pi}(p)^{K-2}2t_{k}$

\begin{equation}
\begin{split}
S_{2} & = [\sum_{i = 1}^{K-2} F_{\pi}(p)^{i}(t_{\#}-it_{k})(1-F_{\pi}(p))c + F_{\pi}(p)^{K-1}2t_{k}c    ]\\
& *(1-F_{\pi}(p))^{\frac{(t_{s}-t_{\#})}{t_{k}}+2}  \\
&=  [ F_{\pi}(p)P_{0}^{K-2} + F_{\pi}(p)^{K-1}2t_{k}c    ](1-F_{\pi}(p))^{\frac{(t_{s}-t_{\#})}{t_{k}}+2}
\end{split}
\end{equation}



\item ...
\item When $t_{m}= t_{s}-t_{k}$, then no matter the job is interrupted by the system or not, the job should stop because of the deadline, where the penalty is 

\begin{equation}
\begin{split}
S_{K-1} & = (1-F_{\pi}(p))^{ \frac{t_{s}-t_{k}}{t_{k}} }cF_{\pi}(p)(t_{\#}-t_{k})  \\
&=  [F_{\pi}(p)P_{0}^{1} + F_{\pi}(p)^{2}(t_{\#}-t_{k})c](1-F_{\pi}(p))^{\frac{t_{s}}{t_{k}}-1}
\end{split}
\end{equation}

\end{itemize}


Note that 

$$P_{0}^{K}  =Kt_{k}-\frac{ct_{k}}{1-F_{\pi}(p)}+\frac{ ct_{k}F_{\pi}(p)^{K}  }{1-F_{\pi}(p)}$$

Considering the above possibilities in (2), the total penalty is:

\begin{equation}
\begin{split}
P_{2} & =S_{1}+S_{2}...+S_{K-1}   \\
& = F_{\pi}(p) (1-F_{\pi}(p))^{  \frac{t_{s} - t_{\#}}{t_{k}}   }\sum_{i = 1}^{K-1}c t_{\#}(1-F_{\pi}(p)  )^{i} \\
& + F_{\pi}(p)(1-F_{\pi}(p))^{ \frac{   t_{s}-t_{\#}}{t_{k}}}(-\frac{ct_{k}}{1-F_{\pi}(p)}) \sum_{i=1}^{K-1} (1-F_{\pi}(p))^{i}+ \\
& F_{\pi}(p)(1-F_{\pi}(p))^{ \frac{   t_{s}-t_{\#}}{t_{k}}}(\frac{ct_{k}}{1-F_{\pi}(p)}) \sum_{i=1}^{K-1} F_{\pi}(p)^{K}(\frac{1-F_{\pi}(p)}{F_{\pi}(p)} )^{i}\\
& -  F_{\pi}(p) (1-F_{\pi}(p))^{  \frac{t_{s} - t_{\#}}{t_{k}}   }\sum_{i = 1}^{K-1}cit_{k}F_{\pi}(p)^{K}( \frac{1-F_{\pi}(p)}{F_{\pi}(p)}  )^{i}\\
&  +(1-F_{\pi}(p))^{  \frac{t_{s} - t_{\#}}{t_{k}}   }ct_{k}F_{\pi}(p)^{K+1} \sum_{i=1}^{K-1}i ( \frac{1-F_{\pi}(p)}{F_{\pi}(p)}  )^{i}\\
& = cF_{\pi}(p)(1-F_{\pi}(p))^{\frac{t_{s}-t_{\#}}{t_{k}}}(t_{\#}- \frac{t_{k}}{1-F_{\pi}(p)})\sum_{i = 1}^{K-1}(1-F_{\pi}(p)  )^{i} \\
& + cF_{\pi}(p)(1-F_{\pi}(p))^{\frac{t_{s}-t_{\#}}{t_{k}}}F_{\pi}(p)^{K} \frac{t_{k}}{1-F_{\pi}(p)}\sum_{i=1}^{K-1}( \frac{1-F_{\pi}(p)}{F_{\pi}(p)}  )^{i}\\
& =  c(1-F_{\pi}(p))^{\frac{t_{s}-t_{\#}}{t_{k}}}(t_{\#}- \frac{t_{k}}{1-F_{\pi}(p)})[  1-F_{\pi}(p) - (1-F_{\pi}(p))^{K}  ]\\
& + c(1-F_{\pi}(p))^{\frac{t_{s}-t_{\#}}{t_{k}}}F_{\pi}(p)^{2}\frac{t_{k}}{1-F_{\pi}(p)}\\
&* \frac{ (1-F_{\pi}(p))F_{\pi}(p)^{K-1}-(1-F_{\pi}(p))^{K}  }{2F_{\pi}(p) -1}\\
& = c(1-F_{\pi}(p))^{\frac{t_{s}-t_{\#}}{t_{k}}}[  t_{\#} ( 1-F_{\pi}(p) - (1-F_{\pi}(p))^{K}   ) \\
& +t_{k} \frac{F_{\pi}(p)^{K+1}}{2F_{\pi}(p) -1}-t_{k} - t_{k} \frac{ (1-F_{\pi}(p))^{K+1}  }{2F_{\pi}(p) -1} ]
\end{split}
\end{equation}


\textbf{(3). Time Line from $t_{s}$ to $+\infty$: the job run on spot instance can not be started}

Because after $t_{s}$, the job will not be started because of the deadline, the total penalty is $$P_{3}= (1-F_{\pi}(p))^{ \frac{t_{s}}{t_{k}}    }c(1-q)t_{e}.$$

The total penalty is $P = P(1) + P(2) + P(3)$.
After some basic calculation, we can get (\ref{penalty}). 
\end{proof}

\begin{claim}\label{cla2}
In persistent request, when $\frac{t_{e}}{2} < t_{s} \leq t_{e}$, $F_{\pi}(p) > 0.5$. 
\end{claim}

Proof of Proposition \ref{pro3}
\begin{proof}
When $\frac{t_{e}}{2} < t_{s} \leq t_{e}$, the decision maker will assign as much job as possible to spot instance to minimize the total cost on the condition that the deadline requirement is met. 

\begin{equation}\label{P3-q}
\begin{split}
q^{*}  =1-\frac{t_{r}+t_{s}F_{\pi}(p)( 1-\frac{t_{r}}{t_{k}}(1-F_{\pi}(p))   )  }{t_{e}}   
\end{split}
\end{equation}

Then substitute $q$ using $q^{*}$ in (P3), we will get a new optimization problem (P3')

\begin{align}
\begin{split}
{\text{(P3') \quad   min}} &
\quad  G(p) = t_{e}\bar{\pi} - t_{r}\bar{\pi} - t_{s}F_{\pi}(p)\bar{\pi}[ 1-\frac{t_{r}}{t_{k}}(1-F_{\pi}(p))] \\
&+t_{s} \int_{\underline{\pi}}^{p}f_{\pi}(x)dx
  \end{split}
\label{green} 
\\
\text{s.t.}\qquad & t_{s}\int_{\underline{\pi}}^{p} xf_{\pi}(x) dx \leq t_{r}\bar{\pi}+t_{s}F_{\pi}(p) \bar{\pi}[1-\frac{t_{r}}{t_{k}}(1-F_{\pi}(p))]
\label{gc0}
\\
&  (1-\frac{t_{r}+t_{s}F_{\pi}(p)( 1-\frac{t_{r}}{t_{k}}(1-F_{\pi}(p))   )  }{t_{e}} ) t_{e} \leq t_{s}
\label{gc1}
\\
& t_{r} < \frac{t_{k}}{1-F_{\pi}(p)}
\label{gc2}
\\
& \underline{\pi} \leq  p \leq \bar{\pi}
\label{gc3}
\\
& 1-\frac{t_{r}+t_{s}F_{\pi}(p)( 1-\frac{t_{r}}{t_{k}}(1-F_{\pi}(p))   )  }{t_{e}}  \geq 0
\label{gc4}
\end{align}

Take the first-order derivative of $G(p)$, we have 
$$ \frac{\partial G(p)}{\partial p}= (p-\bar{\pi})t_{s}f_{\pi}(p) + \frac{t_{r}t_{s}}{t_{k}}\bar{\pi}f_{\pi}(p)(1-2F_{\pi}(p)) <0, $$ so $G(p)$ monotonic decreasing with $p.$ Thus, the optimal solution is $p^{*}= \bar{\pi}$. In addition, the constraints (\ref{gc0}), (\ref{gc1}) and (\ref{gc4}) are satisfied at optimality. 

Substitute $p$ with $p^{*}=\bar{\pi}$ in (\ref{P3-q}), we will get Proposition \ref{pro3}.
\end{proof}


Proof of Proposition \ref{pro4}
\begin{proof}
Similar to the proof of \ref{pro2}, when $t_{s}>t_{e}$, the decision maker will assign the whole job to the spot instance,  i.e., $q=0$. 
\end{proof}



==> strategies_-_1.tex <==


\section{User Bidding Strategies}\label{User Bidding Strategies}

This paper considers the value of portfolio contracts in cloud computing, where users choose to use on-demand and spot instances together to finish a  task. 
By comparing the on-demand price and spot price in \cite{web}, we can see that the spot price is much lower than the on-demand price for every instance type. 
However, the spot market cannot gurantee that the task is run continuously if her bidding price is not high enough, which means the task may be interrupted and takes extra time to get recovered, so that the task may take longer time to get finished. Therefore, the user should balance the propotion of the job she runs on on-demand instance, with the bidding price in an spot market to run the rest job on spot instance. This paper aims to provide a framework to help users decide how much to run at on-demand instances and how to bid for spot instances with the objective to minimizing the total cost, subject to time constraints. 

We consider a series of discrete time slots $t$ and suppose the spot prices $\pi(t)$, $t = 0, 1, ...$ are i.i.d. We use $p$ to denote the user's bid price and $F_{\pi}(p)$ to denote the cumulative distribution function (CDF) of spot price $\pi(p)$, which gives the probability that $p \geq \pi(t)$, i.e., the user's bid is accepted, and the associated probability density function (PDF) is $f_{\pi}(p)$. We also assume that $f_{\pi}(p)$ monotonically decreases, and $F_{\pi}(p)$ is concave. 

Our notations are summarized in Table \ref{tab1}. We not only consider the job's characteristics such as its execution time $t_{e}$, total completion time $T$, the recovery time for writing and transferring the data saved after interruption $t_{r}$, but also include the deadlines on the job completion times. Note that we have three main differences with \cite{lz15}: (1) we add one more decision variable $q$: how much to run on on-demand instance, (2) the required completion time (deadline) $t_{s}$ is added, and (3) bidding strategy for one-time request with penalty is added.

Consider a user faces a certain job $J$, which can be split and run on different instances. The decision consists of two steps. Firstly, facing the job, the user would like to purchase on-demand instances to ensure a certain desired level of finished job in the future; say, $q$ portion of the total amount of task run on on-demand instance. And the rest portion of the job $(1-q)$ will be run on spot instances. Then the user needs to decide how much to bid  to the spot market. Suppose each job has a specific execution time $t_{e}$, which is linear with the amount of task. It is easy to confirm that the time run on on-demand instance is $q t_{e}$, and the cost spent on on-demand instance is $q t_{e}\bar{\pi}$. 

The problem is to desin an optimal portfolio of contracts and bidding strategy, so that the expected total cost is minimized, subject to time constraints. Then we will investigate the extent of the benefits that can be accrued by managing a portfolio of contracts instead of sticking to on-demand instance constract. 

In this section, we first consider one-time requests without penalty, one-time requests with penalty and then persistent requests for a single instance on each machine type. The objectives are to minimize the total cost (including penalty) on the condition that the deadline requirement is satisfied.


\begin{table}[H]
\centering
\caption{Key terms and symbols}
\label{tab1}
\begin{tabular}{|l|l|}
\hline
\textbf{Symbol}   & \textbf{Definition}                                    \\ \hline
$p$               & User bid price                                         \\ \hline
$q$               & The portion of job that will run on on-demand instance \\ \hline
$\pi$             & Spot price                                             \\ \hline
$\bar{\pi}$       & On-demand price                                        \\ \hline
$\underline{\pi}$ & Minimum spot price                                     \\ \hline
$t_{k}$           & Length of one time slot                                \\ \hline
$T$               & Total job completion time                              \\ \hline
$t_{s}$           & Deadline of the job                                    \\ \hline
$t_{e}$           & Job execution time (w/o interruptions)                 \\ \hline
$t_{r}$           & Recovery time from an interruption                     \\ \hline
$c$               & Penalty coefficient                                    \\ \hline
\end{tabular}
\end{table}


\subsection{One-time Requests without Penalty}
In one-time request, part of job will be run on on-demand instance and will not interrupted, and the rest of job will be run on spot instance, where the bidding price falls below the spot price, the job will be terminated and cannot be resumed.

\begin{lemma}
The total cost is $ q t_{e}\bar{\pi} + (1- q)t_{e}\mathbb{E}(\pi | \pi \leq p) $, where $ \mathbb{E}(\pi | \pi \leq p)$ is the expected price that a user must pay to use an instance in each time slot on spot instance or the expected value of all possible spot prices that are no more than $p$ \cite{lz15}: 
$$ \mathbb{E}(\pi | \pi \leq p) = \frac{ \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx}{F_{\pi}(p)}  $$
 
\end{lemma}
 Before we introduce the model, we firstly calculate the expected time to enter the system:

\begin{equation}
t_{n}=t_{k}\sum_{i=1}^{\infty}i (1-F_{\pi}(p))^{i}F_{\pi}(p)= t_{k}(\frac{1}{F_{\pi}(p)}-1)
\end{equation}

Then the optimization problem is proposed: 

\begin{align}
\begin{split}
{\text{(P1) \qquad   min}} &
\qquad     q t_{e}\bar{\pi} + \frac{ (1- q)t_{e}  \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx}{F_{\pi}(p)}
  \end{split}
\label{obj1} 
\\[2ex]
\text{subject to}\qquad & (1-q)t_{e} \leq \frac{t_{k}}{1-F_{\pi}(p)} 
\label{P1-1} 
\\
& q t_{e} \leq t_{s}
\label{P1-2}
\\
&t_{n}+(1-q)t_{e} \leq t_{s}
\label{P1-3}
\\
& \underline{\pi} \leq  p \leq \bar{\pi}
\label{P1-4}
\\
& 0 \leq q \leq 1
\label{P1-5}
\end{align}


In order to make the problem practical, we assume that $t_{e} \leq 2t_{s}$ such that the job can be finished before deadline.

 Constraint (\ref{P1-1})  represents the expected amount of time that a job will continue running without any interruptions $\frac{t_{k}}{1-F_{\pi}(p)}$ must exceed its required execution time on spot instance \cite{lz15}. Comparing to the problem setting in \cite{lz15}, including deadlines on the job completion times introduce constraints (\ref{P1-2}) and (\ref{P1-3}), which shows that the both of maximum job completion time on each instance including the job execution time and time to enter the system (if any) should not exceed the deadline. 


\begin{proposition}\label{pro1}
When $\frac{t_{e}}{2} < t_{s} \leq t_{e}$, the optimal bid price for a one-time request is
  $$p^{*}=\max \{\psi_{1}^{-1} (t_{k}\bar{\pi}), \psi_{2}^{-1} (0)\},$$ where $\psi_{1}^{-1}(.)$ is the inverse function of 
$$\psi_{1}(p)  =\frac{ 2t_{k} \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx  }{  F_{\pi}(p) } + 2pt_{s}F_{\pi}(p) - pt_{s} - (t_{s}+t_{k}) \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx$$ and $\psi_{2}^{-1}(.)$ is the inverse function of 
 $$ \psi_{2}(p)  =   (t_{s}+t_{k})F_{\pi}(p) - (t_{s}+t_{k})F_{\pi}(p)^{2} - t_{k} $$ with $F_{\pi}(p) \geq \frac{1}{2}$. 

And the optimal portion of the job to run on on-demand instance is 
$$   q^{*} = 1- \frac{  t_{s}-t_{k}( \frac{1}{F_{\pi}(p^{*})} -1  )   }{t_{e}}   $$
\end{proposition}

\begin{proposition}\label{pro2}
When $ t_{s} > t_{e}$, the optimal bid price for a one-time request is
  $$p^{*}=F_\pi^{-1}(1-\frac{t_{k}}{t_{e}}).$$ And the optimal portion of the job to run on on-demand instance is 
$$   q^{*} = 0 $$
\end{proposition}

\subsection{One-time Request with Penalty}

Suppose if the job with one-time request assigned to a spot instance is interrupted, there is a penalty $c$ $(c<\bar{\pi})$ for each uncompleted unit job, which is measured by unit time. We denote the time to enter the system as $t_{m}$, $K = \frac{(1-q)t_{e}}{t_{k}}$ and $t_{\#}=(1-q)t_{e}$. So the objective becomes to minimize the total cost for running the job and the penalty for uncompleted job. We begin by finding the expected total penalty and then present the optimization model before deriving the user's optimal bid price. 

\begin{theorem}
With bidding price $p$, the expected unfinished job  is 
\begin{equation}\label{penalty}
\begin{split}
P &= \frac{t_{k}}{2F_{\pi}(p) -1}(1-F_{\pi}(p))^{ \frac{t_{s}}{t_{k}} +1  }[\frac{F_{\pi}(p)^{K}}{(1-F_{\pi}(p))^{K}  }-1]\\
 &+ Kt_{k} + \frac{t_{k}}{1-F_{\pi}(p)}[F_{\pi}(p)^{K}-1]
\end{split}
\end{equation}

\end{theorem}

The optimization problem (P1) becomes 

\begin{align}
\begin{split}
{\text{(P2) \qquad   min}}  \quad &    q t_{e}\bar{\pi} +  ((1- q)t_{e} - P) \frac{\int_{\underline{\pi}}^{p}x f_{\pi}(x)dx}{F_{\pi}(p)} +cP
\end{split}
\\
\text{subject to}&  \quad (\ref{P1-2}),\quad  (\ref{P1-4}), \quad (\ref{P1-5})
\nonumber 
\end{align}

Although the constraints in (P2) are linear, the objective is non-convex. Thus problem (P2) is non-convex. We use the NOVA algorithm proposed in \cite{non}, which is a convex approximation method by solving the optimization problem iteratively. 




\subsection{Persistent Requests}
We now consider a job that places a persistent spot instance request, where the job can be interrupted and recovered upon resuming.
\begin{lemma}
From \cite{lz15}, we know that the expected running time is $TF_{\pi}(p)$ in total completion time $T$ with bidding price $p$, and the associated expected idle time is $(1-F_{\pi}(p))T$. The expected number of idle-to-running transitions in $T/t_{k}$ time slots is $\frac{T}{t_{k}}F_{\pi}(p)(1-F_{\pi}(p))$. Also because $TF_{\pi}(p)=( \frac{T}{t_{k}}F_{\pi}(p)(1-F_{\pi}(p))-1  )t_{r}+(1-q)t_{e}$, we get $TF_{\pi}(p) = \frac{(1-q)t_{e}-t_{r}}{  1- \frac{t_{r}}{t_{k}}(1-F_{\pi}(p))   }$. Therefore, the total time including the recovery, execution and idle time is 

\begin{equation}
\begin{split}
T & = \frac{(1-q)t_{e}-t_{r}}{  1- \frac{t_{r}}{t_{k}}(1-F_{\pi}(p))   }\frac{1}{F_{\pi}(p)}
\end{split}
\end{equation}
\end{lemma}

\begin{align}
\begin{split}
{\text{(P3) \qquad   min}} &
\qquad   q t_{e}\bar{\pi} +\frac{ (1- q)t_{e}-t_{r} }{1-  \frac{t_{r}}{t_{k}} (1-F_{\pi}(p) )   } \frac{ \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx}{F_{\pi}(p)}
  \end{split}
\label{green} 
\\[2ex]
\text{subject to}\qquad &(\ref{P1-2}),\quad  (\ref{P1-4}), \quad (\ref{P1-5})
\nonumber 
\\
&  q t_{e}\bar{\pi} +\frac{ (1- q)t_{e}-t_{r} }{1-  \frac{t_{r}}{t_{k}} (1-F_{\pi}(p) )   } \frac{ \int_{\underline{\pi}}^{p}x f_{\pi}(x)dx}{F_{\pi}(p)} \leq te\bar{\pi}
\label{gc}
\\
&   \frac{(1-q)t_{e}-t_{r}}{  1- \frac{t_{r}}{t_{k}}(1-F_{\pi}(p))   }\frac{1}{F_{\pi}(p)}  \leq t_{s} 
\label{green-constraint-1} 
\\
& t_{r} < \frac{t_{k}}{1-F_{\pi}(p)}
\label{green-constraint-20}
\end{align}

The expected total time including the recovery, execution and idle time should be smaller than the deadline, so we get constraint (\ref{green-constraint-1}). We also take (\ref{green-constraint-20}) as constraint to guarantee the recovery time is sufficiently small such that the job's running time is finite \cite{lz15}. 

\begin{proposition}\label{pro3}
When $\frac{t_{e}}{2} < t_{s} \leq t_{e}$, the optimal bid price for a persistent request is
  $$p^{*}=\bar{\pi}$$ 

And the optimal portion of the job to run on on-demand instance is 
$$   q^{*} = 1- \frac{ t_{r}+t_{s}  }{t_{e}}   $$
\end{proposition}

The Proposition \ref{pro3} thus implies that the bidding price dose not change as the deadline changes, and the optimal portion of the job that run on on-demand instance is decreasing with the deadline. 

\begin{proposition}\label{pro4}
When $ t_{s} > t_{e}$, the optimal bid price for a one-time request is
  $$p^{*}=\psi_{2}^{-1} ( \frac{t_{e}-t_{r}}{t_{s}}  ).$$ 

where $\psi_{2}^{-1}(.)$ is the inverse function of 

$$  \psi_{2}(p) = F_{\pi}(p)[ 1-\frac{t_{r}}{t_{k}}(1-F_{\pi}(p))] $$



And the optimal portion of the job to run on on-demand instance is 
$$   q^{*} = 0 $$
\end{proposition}






